Retrieval Augmented Code Generation and Summarization

Software developers write a lot of source code and documentation during software development. Intrinsically, developers often recall parts of source code or code summaries that they had written in the past while implementing software or documenting them. To mimic developers' code or summary generation behavior, we propose a retrieval augmented framework, REDCODER, that retrieves relevant code or summaries from a retrieval database and provides them as a supplement to code generation or summarization models. REDCODER has a couple of uniqueness. First, it extends the state-of-the-art dense retrieval technique to search for relevant code or summaries. Second, it can work with retrieval databases that include unimodal (only code or natural language description) or bimodal instances (code-description pairs). We conduct experiments and extensive analysis on two benchmark datasets of code generation and summarization in Java and Python, and the promising results endorse the effectiveness of our proposed retrieval augmented framework.

==> tables/input_output.tex <==
\begin{table*}[!ht]
\centering
\resizebox{\linewidth}{!}{
% \small
\def\arraystretch{1.1}%
\begin{tabular}{l|l|l}
\hline
& \tool \coder Input & \coder output \\
& PLBART Encoder Input & PLBART Decoder Input \\
\hline
\multirow{2}{*}{Input} & \multirow{2}{*}{\parbox{7.5cm}{
Get the MuxerStream at the given position . }} &  \multirow{2}{*}{\parbox{7.5cm}{{\color{red} <En>} Find the maximum of three numbers}} \\
& & \\ \hdashline
\multirow{2}{*}{G} & \multirow{2}{*}{\parbox{7.5cm}{ public MuxerStream getMuxerStream ( int position ) { if ( muxerStream == null ) { muxerStream = new MuxerStream ( this , position ) ; } return muxerStream ; }
}} & \multirow{2}{*}{\parbox{7.5cm} { {\color{blue} <java>} public int maximum ( int a , int b , int c ) \{ return Math . max ( a , Math . max ( b , c ) ) \}}} \\
& & \\ \hdashline
\multirow{2}{*}{T} & \multirow{2}{*}{\parbox{7.5cm}{ public int maximum ( int a , int b , int c ) \{ return Math . max ( a , Math . max ( b , c ) ) \} {\color{blue} <java>} }} & \multirow{2}{*}{\parbox{7.5cm}{{\color{orange} <python>} def maximum (a , b , c) : NEW\_LINE INDENT return max ( [ a , b , c ] )}} \\
& & \\
\hline
\end{tabular}
}
% \vspace{-2mm}
\caption{Example inputs to the encoder and decoder for fine-tuning PLBART on sequence generation tasks: source code summarization (S), generation (G), and translation (T).}
\label{table:i/o}
\vspace{-2mm}
\end{table*}



==> tables/not_used_gen_with_comment.tex <==




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[!ht]
\centering
% \resizebox{\linewidth}{!}{%
\small
% \scriptsize
% \def\arraystretch{1.1}%
% \setlength{\tabcolsep}{5pt}
\begin{tabular}{l|c c c| c c c }
\hline
\multirow{ 2}{*}{Methods} & \multicolumn{3}{c|}{CodeXGLUE (Java)} &  \multicolumn{3}{c}{CodeXGLUE (Python)}  \\ 
\cline{2-7}
& BLEU & EM & CodeBLEU & BLEU & EM & CodeBLEU  \\
\hline
\tool (w/o ref) & {26.92} & {8.95} & {31.15} & { 22.74} & {8.88} & {28.93}  \\
\tool (w/o ref with summery) & {\bf 28.98} & {\bf 10.21} & {\bf 33.18} & {\bf 24.43} & {\bf 9.61} & {\bf 30.21} \\
\hline 
\tool (with ref) & 36.33 & {29.41} & {41.38} & {32.14} & {27.48} & {38.02 }  \\
\tool (with ref with summery) & {\bf 42.82} & {\bf 36.99} & {\bf 47.25} &  {\bf 38.87} & {\bf 34.51} & {\bf 43.78} \\
\hline
\end{tabular}
% }
\caption{
Results on source code generation using the retrieved code and its summary together when the reference target code is absent and present in the retrieval database respectively.  
}
% }
\label{table:code_translation}
\vspace{-2mm}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



